ShapeSearch: A Flexible and Efficient System for Shape-based Exploration of Trendlines

Identifying trendline visualizations with desired patterns is a common and fundamental data exploration task. Existing visual analytics tools offer limited flexibility and expressiveness for such tasks, especially when the pattern of interest is under-specified and approximate, and do not scale well when the pattern searching needs are ad-hoc, as is often the case. We propose ShapeSearch, an efficient and flexible pattern-searching tool, that enables the search for desired patterns via multiple mechanisms: sketch, natural-language, and visual regular expressions. We develop a novel shape querying algebra, with a minimal set of primitives and operators that can express a large number of ShapeSearch queries, and design a natural-language and regex-based parser to automatically parse and translate user queries to the algebra representation. To execute these queries within interactive response times, ShapeSearch uses a fast shape algebra-based execution engine with query-aware optimizations, and perceptually-aware scoring methodologies. We present a thorough evaluation of the system, including a general-purpose user study, a case study involving genomic data analysis, as well as performance experiments, comparing against state-of-the-art time series shape matching approaches---that together demonstrate the usability and scalability of ShapeSearch.

==> arch.tex <==
\subsection{System Overview and Usage Scenario}
\label{sec:arch}

%In this section, we first present an overview of the \ssr system along with the user experience.

\ssr  provides a powerful yet flexible mechanisms for users to search for trendline visualizations with a desired shape. Figure~\ref{fig:interface} depicts the \ssr interface, with an example query on genomics data discussed in the introduction. Here, a user is interested in searching for genes that get suppressed due to the influence of a drug, depicted by a specific shape in their gene expression --- first rising, then going down, and finally rising again --- with three patterns: up, down, and up, in a sequence. 

\stitle{Generating Trendline Visualizations}. To search for this shape, the user first loads the dataset~\cite{bult2008mouse}), via form-based options on the left (Figure~\ref{fig:interface} Box 1), and then selects the space of trendline visualizations to explore by setting the visual parameters: $x$ axis as time, the $y$ axis as expression values, and the category ($z$ axis) as gene. \ssr generates a trendline visualization for each unique value of $z$ axis.  Thus, the $z$ axis defines the space of visualizations over which we match the shape.

\stitle{Querying.}  \ssr supports three mechanisms for shape specification: sketching on a canvas, natural language, and regular expressions (regex for short).

\noindent
\emph{Sketching on Canvas}.  By drawing the desired shape as a sketch on the canvas (Figure~\ref{fig:interface} Box 2a), the user can search for visualizations that are \emph{precisely} match (using a distance measure such as Euclidean distance or Dynamic Time Warping~\cite{dtw}).
As soon as the user finishes sketching, \ssr outputs visualizations that are similar to the drawn sketch in the results panel (Figure~\ref{fig:interface} Box 4).

\noindent
\emph{Natural Language (NL)}.
For searching for visualizations that approximately match patterns, users can use natural language.
For instance, as in Figure~\ref{fig:interface}  Box 2b, the desired shape in the aforementioned genomics example can be expressed as \emph{``show me genes that are rising, then going down, and then increasing''}. Similarly, scientists analyzing cosmological data can easily search for supernovae (bright stellar explosions) using 
\emph{``find me objects with a sharp peak in  luminosity''}. We describe in Section~\ref{sec:translation} how \ssr translates natural language queries to a structured internal representation.

\noindent
\emph{Regular Expression (regex)}. For queries that involve complex combinations of patterns 
that are difficult to express using natural language or sketch, the user can issue a regular expression-like query that directly maps to the structured internal representation, consisting of \ssr  primitives and operations, described in detail in Section~\ref{sec:algebra}. 

%During exploration, users can choose specification mechanisms interchangeably based on the complexity of the query. For both NL as well as regex, \ssr, additionally supports auto-complete functionality to guide  users towards their target query. All queries are issued to the back-end using a REST protocol. We use the term \emph{user query} to refer to the submitted query using any of the specification mechanisms.}



%\begin{figure}[htb]
\begin{figure}
\centerline {
\hbox{\resizebox{\columnwidth}{!}{\includegraphics{figs/interface-new.pdf}}}}
\vspace{-2.5pt}
\caption{\smallcaption{\ssr Interface, consisting of six components. 1) Data upload, attributes selection, and applying filter constraints 2) Query specification: 2a)
Sketching canvas 2b) Natural language query interface, and 2c) Regular expression interface, 3) Correction panel, and 4) Results panel}}
\vspace{-13.pt}
\label{fig:interface}
\end{figure}

\stitle{Execution.} The \ssr back-end parses and translates the user query into a \sq, a structured internal representation of the query consisting of operators and primitives supported in our algebra (Section~\ref{sec:algebra}). The back-end supports an ambiguity resolver that uses a set of rules for automatically resolving syntactic and semantic ambiguities, as well as forwards the parsed query to the user for further corrections and validation (Figure~\ref{fig:interface} Box 3). The validated query is finally optimized and executed by the execution engine (Section~\ref{sec:exec}), and the top visualizations that best match the \sq are presented to the user in the results panel (Figure~\ref{fig:interface} Box 4). 
%\papertext{We provide more details on the system in our extended technical report~\cite{techreport}.}


\eat{
\begin{figure}
\centerline {
\hbox{\resizebox{8.5cm}{!}{\includegraphics{figs/nlp_arch.pdf}}}}
\vspace{-4.5pt}
\caption{\smallcaption{System Architecture. \tar{fix}}}
\vspace{-18.5pt}
\label{fig:arch}
\end{figure}
}

==> capabilities.tex <==
%!TEX root = main.tex

\section{Capabilities and Limitations}
\label{sec:capblimitns}


\begin{table}
	\centering
	\caption{Comparison between ShapeSearch and related systems on expressive power over a taxonomy of pattern matching tasks} 
	\label{tab:expressivity}
	\vspace{-8.5pt}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{|l|l|l|l|l|l|}
			\hline 
			Task  & Sketch Systems & Qetch & SDL & \ssr  \\ \hline
			\pbox{4.5cm}{Patterns Supported }  & Precise & Precise & Fuzzy & \pbox{1.5cm}{Precise, Fuzzy}  \\ \hline
			\pbox{3.5cm}{Filtering / Ad hoc  Matching}  & Yes & Yes & No & Yes  \\ \hline
			\pbox{3.5cm}{Range Constraints } & Yes & Yes & No & Yes  \\ \hline
			\pbox{3.5cm}{Sub-Pattern (Range Invariance) Matching}  & \pbox{1.5cm}{Yes (Zenvisage)} & Yes & Yes & Yes  \\ \hline
			\pbox{3.5cm}{Sequence Matching}  & No & No & Yes & Yes   \\ \hline
			\pbox{3.5cm}{Width Selection}  & No & No & No & Yes  \\ \hline
			\pbox{3.5cm}{Multiple X or Y Constraints}   & No & No & No & Yes  \\ \hline
			\pbox{3.5cm}{Quantifiers}  & No & Only repeat & Many & Many  \\ \hline
			\pbox{3.5cm}{Iteration}  & No& No & No & Yes  \\ \hline
			\pbox{3.5cm}{Nesting}  & No& No & No & Yes  \\ \hline
			\pbox{3.5cm}{Backward / Forward Reference} & No& No & No & Yes  \\ \hline
		\end{tabular}%
	}
\end{table}


In previous sections, we  demonstrated how ShapeSearch achieves its two design goals: 1) to enable expressive yet flexible specification of shape search queries, and 2) to facilitate efficient exploration and pattern matching of candidate visualizations. Here, we give brief summary of what ShapeSearch can and cannot do.

As depicted in Table 2, ShapeSearch is sufficiently expressive, covering a taxonomy of pattern matching operations often performed over trendlines.  In particular, one can search for trendlines with precise as well as blurry patterns  with one or more constraints on values, X / Y range, and / or width. A \sq can have a combination of patterns, consisting of  1) a sequence of patterns, 2) conjunction, disjunction, or negation of one or more patterns,  or 3) a pattern with quantifiers such as atleast, at most or between. One can use backward or forward reference to compare two or patterns in the same trendline, iterate over the points in the trendline, group multiple patterns to specify precedence, or use nesting to scope one pattern within the context of another. Besides, \ssr is \emph{extensible} enough such that users can seamlessly add support for new pattern types via user-defined patterns, and either modify existing or add new scoring functions, with the constraint that they satisfy the properties discussed in Section~\ref{sec:exec}.

When configurations such as binning or scale are left unspecified, the \sgt algorithm inherently finds
the best configuration, trying all possible configurations starting from the lowest granularity. Yet, by pruning out less promising visualizations early in the pipeline, \ssr  finds matching visualization within interactive response times.

However, there are few limitations that currently exist in the system. First,  user-defined patterns (e.g.,  periodic patterns), that do not satisfy the properties that our proposed optimizations require, are executed as black-box functions, and hence their execution can be very slow over large datasets. Second, pattern matching is limited to a single visualization at a time,  and therefore ShapeSearch cannot be used for automatically mining insights (e.g., representative trends, outlier trends) over collections of visualizations.




==> cover.tex <==
%!TEX root = main.tex
\vspace{-10pt}

\twocolumn[\section*{Summary of Changes for revised paper --- {\ssr}: A Flexible and Efficient System for Shape-based Exploration of Trendline}]

\vspace{20pt}

We thank the reviewers and the meta-reviewer for their insightful and detailed feedback, and for giving us an opportunity to address their comments. 
We first provide a summary of changes made to the paper, and then respond to the specific points raised in each of the  individual reviews.
All changes to the paper are highlighted in {\color{blue} blue}, and are also referred to in  {\color{blue} blue} in our response below.

%\subsection*{Meta-reviewer Comments}
\stitle{1. More details on performance experiment (Section 5).}  
\rev{We now explain in more detail how we selected queries and ground-truth in Section 5 (see Datasets and setup). We have also replaced the aggregated results with  query-wise results (total 14 in number) in Figure~\ref{fig:perf}.
}

\stitle{2. More details on fuzzy matching.} \rev{We improve the description of fuzzy matching and make it more clear along with the pseudo-code of the algorithm in Section~\ref{sec:fuzzychallenge}}.

\stitle{3. Description of sketching capabilities.} \rev{We now explain in Section 2.3 how a \sq involving sketch is scored. We also explain in detail how a sketch can be optionally used for fuzzy matching in Appendix B in our technical report~\cite{techreport}.}

\stitle{4. Complexity of Line approximation.} \rev{We now elaborate in Section 2.3 as well as present examples from case-study in Section 7.1 that show that even patterns involving complex shapes can be expressed using a small number of lines. In addition, in Sec. 5.2, we evaluate the impact on runtime as we vary the number of lines (i.e., \ssgs in a \concat operation)  from $1$ to $6$.}

\stitle{5. Motivation / need for constraints primtives} \rev{We now explain better the need for constraining timeseries with the help of examples and references to relevant prior work in Section 1.1 (under Ad hoc and Interactive). We also explain how participants applied constraints during the case study in Section 7.}

\stitle{6. Accessibility of algebra}  \rev{We now provide more details and evidence from the user study (that we were earlier described in the technical report) to show that the syntax of visual regex supported by \ssr is easy to learn and use.}

\stitle{7. More details in various sections.} 
\emph{ (i) More examples of queries:} \rev{We now provide additional examples as shown in Table~\ref{tab:examples} in Section 2.1,} \emph{(ii) More details on NL:} 
\rev{We now explain the details on NL more clearly with an example,} \emph{(iii) Protocol and process used:}
\rev{We now refer readers to an earlier published work, where we describe the design study and process in detail. We've currently anonymized the paper for double-blind reasons.}
\emph{(iv) Missing related work:} \rev{We have added the missing related work.}

\stitle{8. Changes for Space.} TODO.


\section{Meta Reviewer}
TODO

%\rcom{M1}{Comment1.}

%\rcom{M2}{Comment 2.}


\section{Reviewer 1}

\rcom{R1.W1, D1}{The paper desperately needs a set of examples of queries to explain the operators and their use.}

\noindent \rev{We now provide additional examples as shown in Table~\ref{tab:examples} in Section 2.1.}


\rcom{R1.W2, D2.}{The underlying assumption is that a line can approximate each pattern in the shape query. This makes sense, but means that complex queries are long queries, involving many concatenated patterns. Understanding how the complexity/length of queries would vary in practice and the effect on results was not clear.}

Line segments have the following advantages: (i) they can efficiently and effectively capture  many shapes, (ii) they are less complex to score and compose, and (iii) they are commonly used in time series for detecting trends.

Even the patterns involving complex shapes often need a small number of features or line segments.  For example, complex shapes (e.g.,  double-bottom, triple-top) in financial domains~\cite{ge1998pattern} can be composed using a maximum of 5 or 6 lines. Even during the case-study on genomics data, we observed that researchers looked for a maximum of $4$ trend changes as part of the same pattern. We found similar results on the analysis of mturk queries. \rev{We now elaborate on these aspects in Section 2.3 as well as Section 7.1}.

\rev{Further, in Sec. 5.2, we evaluate the impact on runtime as we vary the number of lines (i.e., \ssgs in a \concat operation)  from $1$ to $6$.}


\rcom{R1.D3.} {The sketching features are not fully considered, and seem to be a ``me too'' feature. The ``sketch'' primitive is used to match via euclidean or DTW distance for a match, which is exactly what ZenVisage does I believe. Sketching is not mentioned anywhere in scoring as far as I can tell. It is also disabled in the experiments, and sometimes dismissed as unnecessary and other times used to explain why ShapeSeek's results are worse. I found it somewhat disingenuous and irritating to try tountangle what was going on. Moreover, a big motivation for a query algebra is to support multiplequery interfaces with on computational model. So I had thought a sketch would be decomposed intoa concatenation of patterns, perhaps using some simplifications. But this needs to be done carefully to avoid long, complex pattern match queries that would be expensive to evaluate}

\rev{We now explain in Section 2.3 how a \sq involving sketch is scored.}  Since the scoring is quite similar to prior systems, we limit our discussion on precise matching and focus mostly on approximate / fuzzy matching which is the main contribution of our work.
	
In additiona, while sketch is mainly used for precise matching, ShapeSeek optionally allows fuzzy matching via sketch. In order to do so, \ssr first approximates a drawn sketch with a minimal number of lines that users can increase/decrease via a slider and the translates it into a regex. \rev{We now explain approximate matching using a sketch in detail in Appendix B in the technical report.} We currently do not mention this (plus other features of system) in the paper as they do not add to core ideas. For example, an approximate query  expressed using sketch can be directly written using regex.



	
\rcom{R1.D4.}{We find that complex patterns that involve fuzzy patterns and location constraints are easier to describe using NL and regex than to sketch. I can see that there is a potential benefit to this approach when there are lots of fiddly constraints to express. But it's not obvious to me when and where these fiddly constraints arise in practice. I think the case study is compelling, and some of the quotes from the user study are compelling, but it's not clear when the complex constraints dominate the requirements.}

\rev{We now explain better the the need for constraining timeseries with the help of examples as well as with references to relevant prior work in Section 1.1 (under Ad hoc and Interactive). We also explain how participants applied constraints during the case study on genomic dataset in Section 7.} In particular, many prior work have highlighted the usefulness of constraining timeseries pattern search on x and y ranges (e.g., TimeSearcher). Simple examples include, e.g., stock prices / house prices rising or falling within specific ranges of values. In our case study, researchers applied constraints on X and Y axis to compare expression in genes with over similar duration / similar values.  We are happy to motivate this better in our revision.   Also, note that even fuzzy patterns, involving simple shapes such as up / down  without location constraints, are much easier to specify using NL or regex than sketch.

%   has not been proposed before. In addition, optimizer integration and resource-awareness ...\\
%We could re-emphasize our two key questions --- We investigate two major questions in this paper: (1) could we learn accurate, yet {\it robust}, cost models for big data workloads that are much more prone to estimation errors, and (2) could we integrate the learned within the query optimizer and produce both query and resource optimal plans. ... we could focus on the integration part a bit here ..

\rcom{R1.W3. Experiments don't explain/show the queries}

\rev{We now explain in more detail how we selected queries in Section 5 (see Datasets and setup), and that we use results from exhaustive / DP as ground truth as they both are optimal.}
Earlier in Figure 5, we showed aggregated results across all queries for each dataset due to space constraints, \rev{we now add add query-wise results (total 14 in number) in Figure~\ref{fig:perf}}.
Notably, query-wise results are similar to the aggregated results, i.e, for each query the latency of DP (O($n^2$)) is several times worse than the SegmentTree (O(n)) in Figure 5a, and similarly the accuracy of Greedy is much worse than SegmentTree in Figure 5b.
	
\section{Reviewer 2}
\rcom{R2.W1,D2}{There were a few times where I was confused about how the fuzzy matching algorithms work. For example for Step 1 of the SegmentTree Algorithm, I don't understand why there can be $k^2$ subsequences that lie completely in A, for a CONCAT operation with k operands. In general, including more explicit algorithms (like Algorithm 1) would be helpful. Or at least more explanation. }

\rev{We improve the description of fuzzy matching and make it more clear along with the pseudo-code of the algorithm in Section~\ref{sec:fuzzychallenge}}. Regarding ``$k^2$ subsequences in A'', we meant --- for a  CONCAT operation of K operands, there can be $k^2$ possible subsequence, and we score each one of them in A. \rev{We now make it more clear}.

\rcom{R2.W2, D2}{There are not enough details about how the NLI works ... Though the extended report does technically include a few more details for the natural languagepart of the interface, I feel this section is underspecified. For example, I would have liked to seesome of the actual queries collected, or a detailed example of how a specific NL query is mapped to a visual pattern query. I just did not get a good sense of how this component worked from readingthis section of the paper.}

\rev{We now explain the details on NL more clearly with an example.}

\rcom{R2.D3a}{ In general, Section 5 seemed to lack significant detail, and I struggled to understand the significance of the results presented. For example, how were the queries selected for the performance valuations in Section 5? How was the ground truth collected for the accuracy evaluation in 5.1?}
	
\rev{We now explain the experiment setup in more details, as well as replace the aggregate results with query-wise results.} Also, please see our response to R1.W3.
	
\rcom{R2.D3b}{ I just didn't understand the value of Section 5 compared to Section 6.}

In section 6, we evaluate the effectiveness of ShapeSeek w.r.t to other tools on pattern matching tasks involving real users. In contrast, in Section 5, we focus only on ShapeSeek, and compare the runtime and accuracy of our proposed algorithms (DP, Segment-Tree, Greedy) with respect to the exhaustive approach. 
	
\rcom{R2.D3c}{Also, figure 5 is way too small for me to draw any reasonable conclusions, even when viewing it on my computer.}

\rev{We now present query-wise results, and thus got rid of the earlier figure which was showing the aggregated results across all queries.}

\rcom{R2.D1}{I really enjoyed reading about how information was gathered to better understand the use cases and needs of visual query interfaces and languages. This is one of the strongest aspects of the work. If anything, I wish I could hear more about the precise process and protocol used, so others could replicate it. But perhaps this is more appropriate for the technical report.}

Our technical report contains more details on this. In addition, we explain the protocol and process in another related work. \rev{We now cite the paper so that readers can understand the process and protocol better. We've currently anonymized the paper for double-blind reasons.}


\section{Reviewer 3}
\rcom{R3.D2}{ It is unclear how accessible the syntax of the algebra is. It'd be good to have a brief discussionon this in the draft. Also, I'd avoid blown up statements such as ``effortlessly.''}

While one can come up with better ways of issuing or writing the algebraic expressions, it does not affect scoring / execution. That said, \rev{we now provide more details and evidence from the user study (that we were earlier described in the technical report) to show that the syntax of visual regex supported by \ssr is easy to learn and use.} In particular, most of the participants during user study found visual regex (which mimics algebra syntax) easy to learn and use. For example, when asked how easy or difficult it is to learn and apply regex, participants gave a avg. rating of 4.4 out of 5. Moreover, about 2/3rd of the participants said they would opt for regex over natural language or sketch (see Sec. 6: User Preferences and Limitations).

\rcom{R3.D2}{Missing reference; https://people.csail.mit.edu/ tatbul/publications/metrovizsigmod19.pdf}

\rev{We thank the reviewer for pointing this, we now briefly discuss this along with another similar work on time series analytics.}




==> userstudy-techreport.tex <==
%!TEX root = main.tex
\section{User Study}
\label{sec:userstudy}

We conducted a user study to evaluate the utility of \ssr (relative to visual query systems~\cite{zenvisagevldb,timesearcher,googlecorrelate}) on its ability to effectively support pattern matching tasks in trendlines. We also wanted to understand which tasks are easier to express in each of the specification mechanisms:  sketch, natural language, and regular expression. 
We first describe the user study methodology, followed by our key findings from the study.
In the next section, we present a case study with  bioinformatics researchers working on genomics data for a more open-ended evaluation of the tool.

\begin{table}
	\parbox{.48\linewidth}{
		\centering
		\caption{\smallcaption{Overall Results}}
		\vspace{-10pt}
		\resizebox{0.45\columnwidth}{!}{%
		\label{tab:overall_study_quant}
	    	\begin{tabular}{|l|l|l|l|}
			\hline 
			Tool & 	\pbox{1.4cm}{Average Accuracy}    &  \pbox{1.2cm}{Average Time} \\ \hline
				\pbox{2cm}{VQS \\ (only sketch)} & 71\%&	184s\\ \hline
			\pbox{2cm}{\ssrc (NL or regex)} & 88\%	& 105s \\ \hline
		\end{tabular}
		}
	}
	\hfill \hfill \hspace{2pt}
	\parbox{.48\linewidth}{
		\centering
		\caption{\smallcaption{Preferences}}
		\vspace{-10pt}
		\resizebox{0.48\columnwidth}{!}{%
		\label{tab:overall_study_pref}
	 	\begin{tabular}{|l|l|}
			\hline 
			Interface & Preference  \\ \hline
			\pbox{2.5cm}{VQS  \\ (sketch)} &  1/12 \\ \hline
			\pbox{2.5cm}{\ssrc \\ (NL and regex)} & 4/12 \\ \hline
			\pbox{2.5cm}{\ssr  \\ (sketch, NL, and regex together)} & 7/12 \\ \hline
		\end{tabular}%
		}
	}
	\vspace{-10pt}
\end{table}


\eat{
\begin{table}[h]
\centering
\caption{\smallcaption{Overall Results}}
\vspace{-4.5pt}
\label{tab:overall_study_quant}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline 
Tool & Avg Accuracy (\%)   &  Avg Task Completion Time (s) \\ \hline
VQS (only sketch) & 71 &	184 \\ \hline
\ssrc (NL or regex) & 88	& 105 \\ \hline
\end{tabular}%
}
\end{table}
\\


\begin{table}[h]
	\centering
	\caption{\smallcaption{User Preferences for Querying Options}}
	\vspace{-4.5pt}
	\label{tab:overall_study_pref}
	\resizebox{0.7\columnwidth}{!}{%
		\begin{tabular}{|l|l|}
			\hline 
			Interface & Preference  \\ \hline
			VQS (only sketch) &  1/12 \\ \hline
			\ssrc ( only NL and regex) & 4/12 \\ \hline
			\ssr (sketch, NL, and regex together) & 7/12 \\ \hline
		\end{tabular}%
	}
\end{table}
}
\eat{
\stitle{Methodology.} Due to space constraints, we only provide  a brief summary of the methodology here, and refer readers to our extended technical technical report~\cite{techreport} for complete details. (Participants) We conducted the user study using a within-subjects study design with 12 participants (7 male, 5 female) with varying degrees of expertise in data analytics  recruited via flyers and mass-emails.  (Baseline) We developed a baseline tool that replicated the capabilities of visual qyerying systems with a styling scheme identical to the \ssr tool to control for external factors. (Tasks and Datasets) Based on the case studies that served domains we discussed in Introduction, as well as drawing on time series and pattern recognition papers from the data mining~\cite{ralanamahatana2005mining,ye2009time,fu2011review,olszewski2001generalized,han2011data} and visualization community~\cite{2017-regression-by-eye,correll2016semantics,zenvisagevldb,timesearcher,googlecorrelate}; we identified seven subcategories of pattern matching tasks, described in detail in our technical report:
1) Exact trend (ET) , 2) Complex Shape (CS), 3) Sequence Match (SQ), 4) Trend Characterization (TC), 5) Sub-pattern or motif match (SP), 6) Width-specific Match (WS), and 7) Multiple X or  Y Constraints (MXY).
Participants performed these tasks on two real-world datasets: the Weather and the Dow Jones stock datasets from the UCI repository~\cite{ucirepo} (that they could easily understand and relate to), and answered between $3$ to $5$ visualizations that were most relevant to the task. Participants also completed surveys and answered open-ended questions that measured the strengths and weaknesses of the interfaces and the usefulness of the tools in participants' daily work. We also measured the 1) \emph{Task completion time}: the time taken by the participant to provide the their answers for the task, and 2) \emph{Task accuracy} using a ground-truth as follows: (sum of the scores of the visualizations  answered by the participant)*100 / (sum of the scores of the visualizations in the ground-truth).
}

\subsection{User Study Methodology}
\stitle{Participants.} We recruited 12 participants (7 male, 5 female) with varying degrees of expertise in data analytics via flyers and mass-emails. Out of the 12 participants, 7 were graduate students, 3 were undergraduate students, 1 was a  post-doctorate scholar, and 1 was an university employee. While all the participants reported working weekly with data or visualizations (e.g., using excel), 9 out of the 12 participants had prior experience in programming languages (e.g., R, Python, Pandas, and MATLAB), and 5 participants had used SQL before.

\begin{figure}[htb]
\centerline {
\hbox{\resizebox{7.5cm}{!}{\includegraphics{figs/baseline.pdf}}}}
\caption{Baseline Interface \tar{TECHREPORT}}
\vspace{-8.5pt}
\label{fig:baseline}
\end{figure}


\begin{table*}
\centering
\caption{Pattern Matching Tasks \tar{TECHREPORT}} 
\label{tab:study_tasks}
\vspace{-8.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline 
Tasks  & Description (Example Queries)  &  Symbol \\ \hline
Exact Trend Matching &  \pbox{16cm}{Find shapes similar to a specific shape (cities with weather patterns similar to that of NY, stock trends similar to Google's)}    & ET   \\ \hline
Sequence Matching	&  \pbox{16cm}{Find shapes with similar trend changes over time (cities with following temperature trends over time: rise, flat, and fall, stocks with decreasing and then rising trends)}  & SQ   \\ \hline
Sub-pattern matching & \pbox{16cm}{Find frequently occurring sub-pattern (or motif) (stocks that depicted a common sub-pattern found in stocks of Google and Microsoft, cities with $2$ peaks in temperature over the year)} & SP \\ \hline
 Width specific matching & \pbox{16cm}{Find shapes occurring over a specific window (cities with maximum rise or fall in temperature over $3$ months, peaks with a width of $4$ months)} & WS \\ \hline
 Multiple X or Y constraints & \pbox{16cm}{Find shapes with patterns over multiple disjoint regions of the visualization. (stocks with prices rising in a range of 30 to 60 in march, then falling in the same range over the next month)} & MXY \\ \hline
 Trend Characterization & \pbox{16cm}{Summarizing common trends (e.g., find cities with typical weather patterns, stock with typical price patterns)} & TC \\ \hline
 Complex Shape Matching & \pbox{16cm}{Find shapes involving trends along specific directions, and occurring over varying duration (stocks with head and shoulder pattern, cup-shaped patterns, W-shaped patterns)} & CS \\ \hline
\end{tabular}%
}
\end{table*}

\stitle{Baseline.} For the purposes of our study, we explicitly wanted to do a head-to-head qualitative and quantitative comparison of \ssr tool, primarily the natural language and regular expression interfaces, with visual query systems that support a sketch-based querying mechanism for searching for shapes. Thus, we developed a baseline tool, depicted in Figure~\ref{fig:baseline}, that replicated the capabilities of these systems with a styling scheme identical to the \ssr tool to control for external factors. The baseline tool allows users to specify the $x$-axis attribute, $y$-axis attribute, and filters; sketch pattern on a canvas, choose the shape matching measure; zoom in and out of the visualization to focus on specific regions of the visualization; and apply smoothing to match visualizations at varying granularities. On the other hand, we disabled the sketching capability in \ssr for a fairer comparison. \ssrc denotes \ssr with only NL- and regex-based querying mechanisms. 

\stitle{Dataset and Tasks.}
Based on the case studies that served domains we discussed in Introduction, as well as drawing on time series and pattern recognition papers from the data mining~\cite{ralanamahatana2005mining,ye2009time,fu2011review,olszewski2001generalized,han2011data} and visualization community~\cite{2017-regression-by-eye,correll2016semantics,zenvisagevldb,timesearcher,googlecorrelate}; we identified seven subcategories of pattern matching tasks, as depicted in Table~\ref{tab:study_tasks}. \tar{Fix} We designed these tasks on two real-world datasets: the Weather and the Dow Jones stock datasets from the UCI repository~\cite{ucirepo} that participants could easily understand and relate to.  Together the seven tasks touched upon both exploratory search as well as direct / specific pattern-based data exploration, which helped us better gauge the effectiveness of individual interfaces.

\stitle{Study Protocol.}
We conducted the user study using a within-subjects study design, in three phases. First, participants were provided a 15-minute tutorial-cum practice session per tool to get familiarized before performing the tasks. Next, we asked the participants to perform the aforementioned tasks with the orders of the two tools and tasks randomized to reduce any order effects. Participants had to answer between $3$ to $5$ visualizations that were most relevant to the task. Finally, we asked the participants to complete a survey and answer open-ended questions that measured 1) their satisfaction levels, and  preferences among the three interfaces for each of the task, 2) strengths and weaknesses of the interfaces; and 3) usefulness of the tools in participants' daily work. 

\stitle{Ground Truth.} For each of the tasks, three of the authors
%experts with prior experience in visualizations and time series
assigned a score in a range of $0$ (worst match) to $5$ (best match) for each of the candidate visualizations for the tasks. We took the average of the three scores to rate the participants answers. 

\stitle{Metrics.} From data that we recorded during the study, we collected the following metrics: 1) \emph{Task completion time}: the time taken by the participant to provide the their answers for the task. 2) \emph{Task accuracy}: (sum of the scores of the visualizations  answered by the participant)*100 / 
(sum of the scores of the visualizations in the ground-truth). 
3) \emph{Preferences} among the three interfaces, and between the tools for individual tasks as well as overall.
4) \emph{Satisfaction level} with the two tools on a 5-point Likert scale.
In addition, we also analyzed open-ended subjective answers given by participants during the interview sessions. 


\subsection{Key Findings}

\begin{figure*}
	\centering
	\subfloat[Task Accuracy]{\label{fig:study-accuracy}{\includegraphics[width=5.65cm]{figs/studyaccuracy.pdf}}}
	\subfloat[Task Completion Time]{\label{fig:study-time}{\includegraphics[width=5.65cm]{figs/studyresponsetime.pdf}}}
	\subfloat[User Preferences]{\label{fig:study-preference}{\includegraphics[width=5.65cm]{figs/studypreference.pdf}}}
	\vspace{-8.5pt}
 	\caption{User Study Results}
	\vspace{-8.5pt}
\end{figure*}


\cut{
	\begin{figure}[htb]
		\centerline {
			\hbox{\resizebox{8.5cm}{!}{\label{fig:study-accuracy}\includegraphics{figs/studyaccuracy.pdf}}}}
		\vspace{-9.5pt}
		\caption{\smallcaption{Average Accuracy Per Task (error bars indicate standard deviation)}}
		\vspace{-8.5pt}
		\label{fig:study-accuracy}
	\end{figure}
	
	\begin{figure}[htb]
		\centerline {
			\hbox{\resizebox{8.5cm}{!}{\label{fig:study-accuracy}\includegraphics{figs/studyresponsetime.pdf}}}}
		\vspace{-9.5pt}
		\caption{\smallcaption{Average Task Completion Time Per Task
				(error bars indicate standard deviation)}}
		\vspace{-8.5pt}
		\label{fig:study-time}
	\end{figure}
	
	\begin{figure}[htb]
		\centerline {
			\hbox{\resizebox{7.5cm}{!}{\label{fig:study-accuracy}\includegraphics{figs/studypreference.pdf}}}}
		\vspace{-4.5pt}
		\caption{\smallcaption{User Preferences}}
		\vspace{-8.5pt}
		\label{fig:study-preference}
	\end{figure}
}

Now, we describe the key findings from our analysis of the metrics collected during the study. 

\stitle{How accurate were particpants' answers using \ssr and VQS? How long did it take them to finish the tasks?}  As depicted in Table~\ref{tab:overall_study_quant}, \ssrc helps participants achieve higher accuracy (87\%) over VQSs (70\%) in about 40\% less time, a significant improvement both in accuracy and task completion times. While the visual query system involves less reasoning during the query synthesis, it often leads to significantly more manual browsing of candidate visualizations for identifying the desired ones. \ssr, on the other hand, is able to accept more fine-grained user input, and rank relevant visualizations higher, enabling participants to retrieve more accurate answers with less effort.

\cut{
\agp{is this a user task?}\tar{rewrote this part to make it a better fit here. I'm also open to moving it to other sections, if that's better.\\}
\stitle{How effective are \ssr scoring functions compared to similarity measures used in VQSs?}

We also made use of the answers collected during the study to compare \ssr scoring functions with the DTW- and Euclidean-based (supported options in VQS) shape scoring approaches on the ground-truth results. Between DTW and Euclidean distance, participants were free to choose the shape-matching measure according to their preference for the task. For \ssr scoring function, we used the DP-based optimal algorithm for ranking visualizations. As depicted in Figure~\ref{fig:study-accuracy} (red bar) \ssr scoring functions have an overall accuracy of about 94\%, with over 90\% accuracy for about 6 out of the 7 tasks. VQS, as discussed earlier, had an accuracy of 70\%. On complex shape matching tasks, \ssr scoring functions have a relatively less accuracy of 81\%, but is still better than the average accuracy of responses provided by the participants while using visual query systems. Note that for participants answers (blue bars in Figure~\ref{fig:study-accuracy}), we used \sgt-based algorithm for ranking visualizations, since the optimal algorithm is too slow (more details in Section~\ref{sec:exp}).
}

\stitle{How \ssr and VQS compare on individual pattern-matching tasks?} In order to better understand the differences between the tools, we analyzed accuracy and latency results on a per-task basis as depicted in Figure~\ref{fig:study-accuracy} and Figure~\ref{fig:study-time} respectively, and compared these results with the user preferences (Figure~\ref{fig:study-preference})  for individual querying mechanism (collected via survey forms and interview questions). Overall, we found that the accuracy and the task completion times are closely related with the expressivity of the tools.  We summarize our findings below.

%\begin{itemize}[noitemsep,parsep=0pt,partopsep=0pt,leftmargin=*]
\emph{More number of participants (9/12) preferred sketch-based querying interface compared to \ssr(7/12) for precise pattern matching tasks} that involved finding visualizations that were exactly similar to a given visualization. Moreover, participants gave more accurate answers in relatively less time while using sketch-based querying.
Participants (4/12) who preferred both mentioned they would use sketch if they want to search for visualizations that had similar values to the given visualization, but would use either NL or Regex if they want to search for high-level changes in trends  over time. 

\emph{While searching for complex shapes (e.g., stocks with double top pattern), more participants (7/12) tend to prefer sketch-based querying, and took less time to complete their tasks compared to \ssr (6/12). However participants had more accurate answers when using \ssr}. Participants believed it is \emph{less effort} to sketch and modify complex shapes on the canvas and select dynamic time warping (DTW) for finding similar shapes, compared to writing a regex. However, \ssr resulted in higher accuracy because the scoring methodology used in \ssr is better at abstracting trends, and more robust to random fluctuations in sequence values than the DTW measure which compares and aligns visualizations solely based on values.

\emph{Majority of the participants (11/12) preferred \ssr for searching visualizations with a sequence or a subsequence of  patterns, and provided more accurate answers in less time}. 
Since visual query systems are based on precise sketch matching, users have to draw multiple sketches for a given sequence or subsequence to find all possible instances. \ssr, on the other, is more effective at automatically finding a variety of shapes that satisfy the same sequence or subsequence of patterns.

\emph{For tasks involving multiple constraints along the X and Y axes, or the width of patterns, a large majority of the participants preferred \ssr, and provided more accurate results in less time}. This is because \ssr supports a rich set of primitives for users to add multiple constraints on the patterns, including searching patterns over multiple disjoint regions. While the users could zoom into a specific region of the visualization and sketch their desired patterns in the visual query system, these capabilities were not sufficient to precisely specify all constraints at the same time. We believe effectively implementing primitives supported by \ssr using visual widgets, and providing effective coordination between the widgets and the canvas is a challenging task, and is an interesting future work.

Overall, when we asked participants which tool they would prefer for pattern matching tasks in their workflow, $11$ out of $12$ participants preferred \ssr (with three interfaces integrated together) over visual query systems. Only $1$ participant considered visual query systems sufficient for her data analysis work, while $4$ participants believed natural and regex together without sketch can be sufficient. Participant P2 said ``\textit{Almost always, I will go with Tool B [\ssrc]. I know exactly what I am searching [for] and what the tool is going to do, it is much more concise, I feel more confident in expressing my query pattern}". On a $5$-point Likert scale ranging from strongly disagree (1) to strongly agree (5), participants rated visual query systems $2.8$ and \ssr $4.2$ when asked about how effectively and flexibly these tools helped them express their intended patterns.


\stitle{Which querying mechanism is more useful between NL and regex?}
Out of $11$ participants who preferred \ssr over visual query systems, $7$ said they would opt for regex over natural language and sketch, if they had to choose one. This was surprising given $5$ of these participants had no prior experience with regular expressions-like languages. Participant P8 said ``\textit{the concept for visual regex by itself is very powerful, could be helpful for most cases in general}''. Participant p4 said ``\textit{Regex was very friendly to use, very powerful for a large number of usecases}''. On the other hand, participant P1 who preferred natural language over regex said, ``\textit{Natural language and drawing [sketching-based querying] are good [sufficient] for most of the patterns, once or twice [rarely] I will search for complicated patterns with constraints, but I can then first use natural language and then fill the missing fields in the [form-based correction] panel below...}"
On a $5$-point Likert scale ranging from strongly disagree (1) to strongly agree (5), participants gave a score of $3.9$ when asked how effective \ssr was in understanding and parsing their natural language queries. And when asked how easy it was to learn and apply regular expression, they gave a rating of $4.2$.

\stitle{How effective is line-segments-based shape matching?} When asked about the effectiveness of using line-segments for approximating and matching trendlines, the average response was positive with a rating of 3.9 on a scale of 5. 
Participant 4 said ``\textit{Green lines [line-segments fitted over the visualization in \ssr] are good, they make me more confident, help me understand visualizations especially [the] noisy ones without me having to spend too much time  parsing signals. I can also see how my [query] pattern was fitted over the visualization ...}''.


\stitle{How can \ssr be improved?}. Participants suggested several improvements to make \ssr more useful in their workflows. A large number of participants wanted \ssr to support more mathematical patterns by default like concave, convex, exponential, or statistical measures such as entropy. For line-segment based approximations, participants suggested we use different colors for lines that correspond to different patterns (\ssgs) in the \sq. Moreover, syntax for regex can be made simpler by removing square brackets, supporting better symbols for primitives and operators,  and supporting more real time regex validation and auto-correction. Finally, a few  participants suggested that we should recommend queries and visualization based on learning from historical queries. \tar{conversation}.

\vspace{-5.5pt}
\subsection{Effectiveness of  Scoring Functions}
\label{subsec:scoringeffectiveness}
We evaluated the effectiveness of \ssr scoring functions compared to DTW- and Euclidean-based (both supported options in VQS) shape similarity measures on the ground-truth results. Since the answers can vary depending on the drawn trendline (sketch) and settings 
(e.g., smoothing) of the VQSs, for Euclidean and DTW, we used the answers provided by participants based on their judgment. Moreover, between DTW and Euclidean, participants were free to choose the option that they felt was more appropriate and relevant to the task.
For \ssr scoring functions, we used the DP-based optimal algorithm for ranking visualizations. Note that during the study, we used \sgt-based algorithm for ranking visualizations  (results depicted via blue bars in Figure~\ref{fig:study-accuracy}), since the optimal algorithm is too slow (discussed in more detail in Section~\ref{sec:exp}). As depicted in Figure~\ref{fig:study-accuracy} (red bar) \ssr scoring functions have an accuracy of over 89\% accuracy for about 6 out of the 7 tasks. VQSs, as discussed earlier, have a comparatively lower accuracy of 71\%. On complex shape matching tasks, \ssr scoring functions have a relatively less accuracy of 81\% than over other tasks, but is still better than the average accuracy of responses provided by the participants while using VQSs.


==> userstudy.tex <==
%!TEX root = main.tex
\section{User Study}
\label{sec:userstudy}

We conducted a user study to evaluate the utility of \ssr (relative to visual query systems~\cite{zenvisagevldb,timesearcher,googlecorrelate}) on its ability to effectively support pattern matching tasks in trendlines. We also wanted to understand which tasks are easier to express in each of the specification mechanisms:  sketch, natural language, and regular expression. 
We first describe the user study methodology, followed by our key findings from the study.
In the next section, we present a case study with  bioinformatics researchers working on genomics data for a more open-ended evaluation of the tool.

\begin{table}
	\parbox{.48\linewidth}{
		\centering
		\caption{\smallcaption{Overall Results}}
		\vspace{-10pt}
		\resizebox{0.45\columnwidth}{!}{%
		\label{tab:overall_study_quant}
	    	\begin{tabular}{|l|l|l|l|}
			\hline 
			Tool & 	\pbox{1.4cm}{Average Accuracy}    &  \pbox{1.2cm}{Average Time} \\ \hline
				\pbox{2cm}{VQS \\ (only sketch)} & 71\%&	184s\\ \hline
			\pbox{2cm}{\ssrc (NL or regex)} & 88\%	& 105s \\ \hline
		\end{tabular}
		}
	}
	\hfill \hfill \hspace{2pt}
	\parbox{.48\linewidth}{
		\centering
		\caption{\smallcaption{Preferences}}
		\vspace{-10pt}
		\resizebox{0.48\columnwidth}{!}{%
		\label{tab:overall_study_pref}
	 	\begin{tabular}{|l|l|}
			\hline 
			Interface & Preference  \\ \hline
			\pbox{2.5cm}{VQS  \\ (sketch)} &  1/12 \\ \hline
			\pbox{2.5cm}{\ssrc \\ (NL and regex)} & 4/12 \\ \hline
			\pbox{2.5cm}{\ssr  \\ (sketch, NL, and regex together)} & 7/12 \\ \hline
		\end{tabular}%
		}
	}
	\vspace{-10pt}
\end{table}


\eat{
\begin{table}[h]
\centering
\caption{\smallcaption{Overall Results}}
\vspace{-4.5pt}
\label{tab:overall_study_quant}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline 
Tool & Avg Accuracy (\%)   &  Avg Task Completion Time (s) \\ \hline
VQS (only sketch) & 71 &	184 \\ \hline
\ssrc (NL or regex) & 88	& 105 \\ \hline
\end{tabular}%
}
\end{table}
\\


\begin{table}[h]
	\centering
	\caption{\smallcaption{User Preferences for Querying Options}}
	\vspace{-4.5pt}
	\label{tab:overall_study_pref}
	\resizebox{0.7\columnwidth}{!}{%
		\begin{tabular}{|l|l|}
			\hline 
			Interface & Preference  \\ \hline
			VQS (only sketch) &  1/12 \\ \hline
			\ssrc ( only NL and regex) & 4/12 \\ \hline
			\ssr (sketch, NL, and regex together) & 7/12 \\ \hline
		\end{tabular}%
	}
\end{table}
}
\eat{
\stitle{Methodology.} Due to space constraints, we only provide  a brief summary of the methodology here, and refer readers to our extended technical technical report~\cite{techreport} for complete details. (Participants) We conducted the user study using a within-subjects study design with 12 participants (7 male, 5 female) with varying degrees of expertise in data analytics  recruited via flyers and mass-emails.  (Baseline) We developed a baseline tool that replicated the capabilities of visual qyerying systems with a styling scheme identical to the \ssr tool to control for external factors. (Tasks and Datasets) Based on the case studies that served domains we discussed in Introduction, as well as drawing on time series and pattern recognition papers from the data mining~\cite{ralanamahatana2005mining,ye2009time,fu2011review,olszewski2001generalized,han2011data} and visualization community~\cite{2017-regression-by-eye,correll2016semantics,zenvisagevldb,timesearcher,googlecorrelate}; we identified seven subcategories of pattern matching tasks, described in detail in our technical report:
1) Exact trend (ET) , 2) Complex Shape (CS), 3) Sequence Match (SQ), 4) Trend Characterization (TC), 5) Sub-pattern or motif match (SP), 6) Width-specific Match (WS), and 7) Multiple X or  Y Constraints (MXY).
Participants performed these tasks on two real-world datasets: the Weather and the Dow Jones stock datasets from the UCI repository~\cite{ucirepo} (that they could easily understand and relate to), and answered between $3$ to $5$ visualizations that were most relevant to the task. Participants also completed surveys and answered open-ended questions that measured the strengths and weaknesses of the interfaces and the usefulness of the tools in participants' daily work. We also measured the 1) \emph{Task completion time}: the time taken by the participant to provide the their answers for the task, and 2) \emph{Task accuracy} using a ground-truth as follows: (sum of the scores of the visualizations  answered by the participant)*100 / (sum of the scores of the visualizations in the ground-truth).
}

\subsection{User Study Methodology}
\stitle{Participants.} We recruited 12 participants (7 male, 5 female) with varying degrees of expertise in data analytics via flyers and mass-emails. Out of the 12 participants, 7 were graduate students, 3 were undergraduate students, 1 was a  post-doctorate scholar, and 1 was an university employee. While all the participants reported working weekly with data or visualizations (e.g., using excel), 9 out of the 12 participants had prior experience in programming languages (e.g., R, Python, Pandas, and MATLAB), and 5 participants had used SQL before.

\begin{figure}[htb]
\centerline {
\hbox{\resizebox{7.5cm}{!}{\includegraphics{figs/baseline.pdf}}}}
\caption{Baseline Interface \tar{TECHREPORT}}
\vspace{-8.5pt}
\label{fig:baseline}
\end{figure}


\begin{table*}
\centering
\caption{Pattern Matching Tasks \tar{TECHREPORT}} 
\label{tab:study_tasks}
\vspace{-8.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline 
Tasks  & Description (Example Queries)  &  Symbol \\ \hline
Exact Trend Matching &  \pbox{16cm}{Find shapes similar to a specific shape (cities with weather patterns similar to that of NY, stock trends similar to Google's)}    & ET   \\ \hline
Sequence Matching	&  \pbox{16cm}{Find shapes with similar trend changes over time (cities with following temperature trends over time: rise, flat, and fall, stocks with decreasing and then rising trends)}  & SQ   \\ \hline
Sub-pattern matching & \pbox{16cm}{Find frequently occurring sub-pattern (or motif) (stocks that depicted a common sub-pattern found in stocks of Google and Microsoft, cities with $2$ peaks in temperature over the year)} & SP \\ \hline
 Width specific matching & \pbox{16cm}{Find shapes occurring over a specific window (cities with maximum rise or fall in temperature over $3$ months, peaks with a width of $4$ months)} & WS \\ \hline
 Multiple X or Y constraints & \pbox{16cm}{Find shapes with patterns over multiple disjoint regions of the visualization. (stocks with prices rising in a range of 30 to 60 in march, then falling in the same range over the next month)} & MXY \\ \hline
 Trend Characterization & \pbox{16cm}{Summarizing common trends (e.g., find cities with typical weather patterns, stock with typical price patterns)} & TC \\ \hline
 Complex Shape Matching & \pbox{16cm}{Find shapes involving trends along specific directions, and occurring over varying duration (stocks with head and shoulder pattern, cup-shaped patterns, W-shaped patterns)} & CS \\ \hline
\end{tabular}%
}
\end{table*}

\stitle{Baseline.} For the purposes of our study, we explicitly wanted to do a head-to-head qualitative and quantitative comparison of \ssr tool, primarily the natural language and regular expression interfaces, with visual query systems that support a sketch-based querying mechanism for searching for shapes. Thus, we developed a baseline tool, depicted in Figure~\ref{fig:baseline}, that replicated the capabilities of these systems with a styling scheme identical to the \ssr tool to control for external factors. The baseline tool allows users to specify the $x$-axis attribute, $y$-axis attribute, and filters; sketch pattern on a canvas, choose the shape matching measure; zoom in and out of the visualization to focus on specific regions of the visualization; and apply smoothing to match visualizations at varying granularities. On the other hand, we disabled the sketching capability in \ssr for a fairer comparison. \ssrc denotes \ssr with only NL- and regex-based querying mechanisms. 

\stitle{Dataset and Tasks.}
Based on the case studies that served domains we discussed in Introduction, as well as drawing on time series and pattern recognition papers from the data mining~\cite{ralanamahatana2005mining,ye2009time,fu2011review,olszewski2001generalized,han2011data} and visualization community~\cite{2017-regression-by-eye,correll2016semantics,zenvisagevldb,timesearcher,googlecorrelate}; we identified seven subcategories of pattern matching tasks, as depicted in Table~\ref{tab:study_tasks}. \tar{Fix} We designed these tasks on two real-world datasets: the Weather and the Dow Jones stock datasets from the UCI repository~\cite{ucirepo} that participants could easily understand and relate to.  Together the seven tasks touched upon both exploratory search as well as direct / specific pattern-based data exploration, which helped us better gauge the effectiveness of individual interfaces.

\stitle{Study Protocol.}
We conducted the user study using a within-subjects study design, in three phases. First, participants were provided a 15-minute tutorial-cum practice session per tool to get familiarized before performing the tasks. Next, we asked the participants to perform the aforementioned tasks with the orders of the two tools and tasks randomized to reduce any order effects. Participants had to answer between $3$ to $5$ visualizations that were most relevant to the task. Finally, we asked the participants to complete a survey and answer open-ended questions that measured 1) their satisfaction levels, and  preferences among the three interfaces for each of the task, 2) strengths and weaknesses of the interfaces; and 3) usefulness of the tools in participants' daily work. 

\stitle{Ground Truth.} For each of the tasks, three of the authors
%experts with prior experience in visualizations and time series
assigned a score in a range of $0$ (worst match) to $5$ (best match) for each of the candidate visualizations for the tasks. We took the average of the three scores to rate the participants answers. 

\stitle{Metrics.} From data that we recorded during the study, we collected the following metrics: 1) \emph{Task completion time}: the time taken by the participant to provide the their answers for the task. 2) \emph{Task accuracy}: (sum of the scores of the visualizations  answered by the participant)*100 / 
(sum of the scores of the visualizations in the ground-truth). 
3) \emph{Preferences} among the three interfaces, and between the tools for individual tasks as well as overall.
4) \emph{Satisfaction level} with the two tools on a 5-point Likert scale.
In addition, we also analyzed open-ended subjective answers given by participants during the interview sessions. 


\subsection{Key Findings}

\begin{figure*}
	\centering
	\subfloat[Task Accuracy]{\label{fig:study-accuracy}{\includegraphics[width=5.65cm]{figs/studyaccuracy.pdf}}}
	\subfloat[Task Completion Time]{\label{fig:study-time}{\includegraphics[width=5.65cm]{figs/studyresponsetime.pdf}}}
	\subfloat[User Preferences]{\label{fig:study-preference}{\includegraphics[width=5.65cm]{figs/studypreference.pdf}}}
	\vspace{-8.5pt}
 	\caption{User Study Results}
	\vspace{-8.5pt}
\end{figure*}


\cut{
	\begin{figure}[htb]
		\centerline {
			\hbox{\resizebox{8.5cm}{!}{\label{fig:study-accuracy}\includegraphics{figs/studyaccuracy.pdf}}}}
		\vspace{-9.5pt}
		\caption{\smallcaption{Average Accuracy Per Task (error bars indicate standard deviation)}}
		\vspace{-8.5pt}
		\label{fig:study-accuracy}
	\end{figure}
	
	\begin{figure}[htb]
		\centerline {
			\hbox{\resizebox{8.5cm}{!}{\label{fig:study-accuracy}\includegraphics{figs/studyresponsetime.pdf}}}}
		\vspace{-9.5pt}
		\caption{\smallcaption{Average Task Completion Time Per Task
				(error bars indicate standard deviation)}}
		\vspace{-8.5pt}
		\label{fig:study-time}
	\end{figure}
	
	\begin{figure}[htb]
		\centerline {
			\hbox{\resizebox{7.5cm}{!}{\label{fig:study-accuracy}\includegraphics{figs/studypreference.pdf}}}}
		\vspace{-4.5pt}
		\caption{\smallcaption{User Preferences}}
		\vspace{-8.5pt}
		\label{fig:study-preference}
	\end{figure}
}

Now, we describe the key findings from our analysis of the metrics collected during the study. 

\stitle{How accurate were particpants' answers using \ssr and VQS? How long did it take them to finish the tasks?}  As depicted in Table~\ref{tab:overall_study_quant}, \ssrc helps participants achieve higher accuracy (87\%) over VQSs (70\%) in about 40\% less time, a significant improvement both in accuracy and task completion times. While the visual query system involves less reasoning during the query synthesis, it often leads to significantly more manual browsing of candidate visualizations for identifying the desired ones. \ssr, on the other hand, is able to accept more fine-grained user input, and rank relevant visualizations higher, enabling participants to retrieve more accurate answers with less effort.

\cut{
\agp{is this a user task?}\tar{rewrote this part to make it a better fit here. I'm also open to moving it to other sections, if that's better.\\}
\stitle{How effective are \ssr scoring functions compared to similarity measures used in VQSs?}

We also made use of the answers collected during the study to compare \ssr scoring functions with the DTW- and Euclidean-based (supported options in VQS) shape scoring approaches on the ground-truth results. Between DTW and Euclidean distance, participants were free to choose the shape-matching measure according to their preference for the task. For \ssr scoring function, we used the DP-based optimal algorithm for ranking visualizations. As depicted in Figure~\ref{fig:study-accuracy} (red bar) \ssr scoring functions have an overall accuracy of about 94\%, with over 90\% accuracy for about 6 out of the 7 tasks. VQS, as discussed earlier, had an accuracy of 70\%. On complex shape matching tasks, \ssr scoring functions have a relatively less accuracy of 81\%, but is still better than the average accuracy of responses provided by the participants while using visual query systems. Note that for participants answers (blue bars in Figure~\ref{fig:study-accuracy}), we used \sgt-based algorithm for ranking visualizations, since the optimal algorithm is too slow (more details in Section~\ref{sec:exp}).
}

\stitle{How \ssr and VQS compare on individual pattern-matching tasks?} In order to better understand the differences between the tools, we analyzed accuracy and latency results on a per-task basis as depicted in Figure~\ref{fig:study-accuracy} and Figure~\ref{fig:study-time} respectively, and compared these results with the user preferences (Figure~\ref{fig:study-preference})  for individual querying mechanism (collected via survey forms and interview questions). Overall, we found that the accuracy and the task completion times are closely related with the expressivity of the tools.  We summarize our findings below.

%\begin{itemize}[noitemsep,parsep=0pt,partopsep=0pt,leftmargin=*]
\emph{More number of participants (9/12) preferred sketch-based querying interface compared to \ssr(7/12) for precise pattern matching tasks} that involved finding visualizations that were exactly similar to a given visualization. Moreover, participants gave more accurate answers in relatively less time while using sketch-based querying.
Participants (4/12) who preferred both mentioned they would use sketch if they want to search for visualizations that had similar values to the given visualization, but would use either NL or Regex if they want to search for high-level changes in trends  over time. 

\emph{While searching for complex shapes (e.g., stocks with double top pattern), more participants (7/12) tend to prefer sketch-based querying, and took less time to complete their tasks compared to \ssr (6/12). However participants had more accurate answers when using \ssr}. Participants believed it is \emph{less effort} to sketch and modify complex shapes on the canvas and select dynamic time warping (DTW) for finding similar shapes, compared to writing a regex. However, \ssr resulted in higher accuracy because the scoring methodology used in \ssr is better at abstracting trends, and more robust to random fluctuations in sequence values than the DTW measure which compares and aligns visualizations solely based on values.

\emph{Majority of the participants (11/12) preferred \ssr for searching visualizations with a sequence or a subsequence of  patterns, and provided more accurate answers in less time}. 
Since visual query systems are based on precise sketch matching, users have to draw multiple sketches for a given sequence or subsequence to find all possible instances. \ssr, on the other, is more effective at automatically finding a variety of shapes that satisfy the same sequence or subsequence of patterns.

\emph{For tasks involving multiple constraints along the X and Y axes, or the width of patterns, a large majority of the participants preferred \ssr, and provided more accurate results in less time}. This is because \ssr supports a rich set of primitives for users to add multiple constraints on the patterns, including searching patterns over multiple disjoint regions. While the users could zoom into a specific region of the visualization and sketch their desired patterns in the visual query system, these capabilities were not sufficient to precisely specify all constraints at the same time. We believe effectively implementing primitives supported by \ssr using visual widgets, and providing effective coordination between the widgets and the canvas is a challenging task, and is an interesting future work.

Overall, when we asked participants which tool they would prefer for pattern matching tasks in their workflow, $11$ out of $12$ participants preferred \ssr (with three interfaces integrated together) over visual query systems. Only $1$ participant considered visual query systems sufficient for her data analysis work, while $4$ participants believed natural and regex together without sketch can be sufficient. Participant P2 said ``\textit{Almost always, I will go with Tool B [\ssrc]. I know exactly what I am searching [for] and what the tool is going to do, it is much more concise, I feel more confident in expressing my query pattern}". On a $5$-point Likert scale ranging from strongly disagree (1) to strongly agree (5), participants rated visual query systems $2.8$ and \ssr $4.2$ when asked about how effectively and flexibly these tools helped them express their intended patterns.


\stitle{Which querying mechanism is more useful between NL and regex?}
Out of $11$ participants who preferred \ssr over visual query systems, $7$ said they would opt for regex over natural language and sketch, if they had to choose one. This was surprising given $5$ of these participants had no prior experience with regular expressions-like languages. Participant P8 said ``\textit{the concept for visual regex by itself is very powerful, could be helpful for most cases in general}''. Participant p4 said ``\textit{Regex was very friendly to use, very powerful for a large number of usecases}''. On the other hand, participant P1 who preferred natural language over regex said, ``\textit{Natural language and drawing [sketching-based querying] are good [sufficient] for most of the patterns, once or twice [rarely] I will search for complicated patterns with constraints, but I can then first use natural language and then fill the missing fields in the [form-based correction] panel below...}"
On a $5$-point Likert scale ranging from strongly disagree (1) to strongly agree (5), participants gave a score of $3.9$ when asked how effective \ssr was in understanding and parsing their natural language queries. And when asked how easy it was to learn and apply regular expression, they gave a rating of $4.2$.

\stitle{How effective is line-segments-based shape matching?} When asked about the effectiveness of using line-segments for approximating and matching trendlines, the average response was positive with a rating of 3.9 on a scale of 5. 
Participant 4 said ``\textit{Green lines [line-segments fitted over the visualization in \ssr] are good, they make me more confident, help me understand visualizations especially [the] noisy ones without me having to spend too much time  parsing signals. I can also see how my [query] pattern was fitted over the visualization ...}''.


\stitle{How can \ssr be improved?}. Participants suggested several improvements to make \ssr more useful in their workflows. A large number of participants wanted \ssr to support more mathematical patterns by default like concave, convex, exponential, or statistical measures such as entropy. For line-segment based approximations, participants suggested we use different colors for lines that correspond to different patterns (\ssgs) in the \sq. Moreover, syntax for regex can be made simpler by removing square brackets, supporting better symbols for primitives and operators,  and supporting more real time regex validation and auto-correction. Finally, a few  participants suggested that we should recommend queries and visualization based on learning from historical queries. \tar{conversation}.

\vspace{-5.5pt}
\subsection{Effectiveness of  Scoring Functions}
\label{subsec:scoringeffectiveness}
We evaluated the effectiveness of \ssr scoring functions compared to DTW- and Euclidean-based (both supported options in VQS) shape similarity measures on the ground-truth results. Since the answers can vary depending on the drawn trendline (sketch) and settings 
(e.g., smoothing) of the VQSs, for Euclidean and DTW, we used the answers provided by participants based on their judgment. Moreover, between DTW and Euclidean, participants were free to choose the option that they felt was more appropriate and relevant to the task.
For \ssr scoring functions, we used the DP-based optimal algorithm for ranking visualizations. Note that during the study, we used \sgt-based algorithm for ranking visualizations  (results depicted via blue bars in Figure~\ref{fig:study-accuracy}), since the optimal algorithm is too slow (discussed in more detail in Section~\ref{sec:exp}). As depicted in Figure~\ref{fig:study-accuracy} (red bar) \ssr scoring functions have an accuracy of over 89\% accuracy for about 6 out of the 7 tasks. VQSs, as discussed earlier, have a comparatively lower accuracy of 71\%. On complex shape matching tasks, \ssr scoring functions have a relatively less accuracy of 81\% than over other tasks, but is still better than the average accuracy of responses provided by the participants while using VQSs.

